No Query, No Access

Textual adversarial attacks mislead NLP models, including Large Language Models (LLMs), by subtly modifying text. While effective, existing attacks often require knowledge of the victim model, extensive queries, or access to training data, limiting real-world feasibility. To overcome these constraints, we introduce the \textbf{Victim Data-based Adversarial Attack (VDBA)}, which operates using only victim texts. To prevent access to the victim model, we create a shadow dataset with publicly available pre-trained models and clustering methods as a foundation for developing substitute models. To address the low attack success rate (ASR) due to insufficient information feedback, we propose the hierarchical substitution model design, generating substitute models to mitigate the failure of a single substitute model at the decision boundary. Concurrently, we use diverse adversarial example generation, employing various attack methods to generate and select the adversarial example with better similarity and attack effectiveness. Experiments on the Emotion and SST5 datasets show that VDBA outperforms state-of-the-art methods, achieving an ASR improvement of 52.08\% while significantly reducing attack queries to 0. More importantly, we discover that VDBA poses a significant threat to LLMs such as Qwen2 and the GPT family, and achieves the highest ASR of 45.99% even without access to the API, confirming that advanced NLP models still face serious security risks. Our codes can be found at https://anonymous.4open.science/r/VDBA-Victim-Data-based-Adversarial-Attack-36EC/

==> sec/0_abstract.tex <==
\begin{abstract}
Textual adversarial attacks confuse Natural Language Processing (NLP) models, such as Large Language Models (LLMs), by finely modifying the text, resulting in incorrect decisions. Although existing adversarial attacks are effective, they typically rely on knowing the victim model, using extensive queries, or grasping training data, which limits their real-world applications. In situations where there is neither knowledge of nor access to the victim model, we introduce the \textbf{Free Lunch Adversarial Attack (FLA)}, demonstrating that attackers can successfully execute attacks armed only with victim texts. To prevent access to the victim model, we create a shadow dataset with publicly available pre-trained models and clustering methods as a foundation for developing substitute models. To address the low attack success rate (ASR) due to insufficient information feedback, we propose the hierarchical substitution model design, generating substitute models that approximate the victim's decision boundaries to enhance ASR. Concurrently, we use diverse adversarial example generation, employing various attack methods to reduce the frequency of model training, balancing effectiveness with efficiency. Experiments with the Emotion and SST5 datasets show that the FLA outperforms existing state-of-the-art methods while lowering the attack cost to zero. More importantly, we discover that FLA poses a significant threat to LLMs such as  Qwen2 and the GPT family, and achieves the highest ASR of 45.99\% even without access to the API, confirming that advanced NLP models still face serious security risks.
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Text classification is a task in natural language processing that organizes and categorizes information by automatically assigning text content to predefined categories or labels~\citep{fields2024survey}.Neural networks have greatly improved the performance of text classification, and these text classification models have become increasingly important, especially after the popularity of large models (LLMs) ~\citep{sun2023text}. However, textual adversarial attacks trigger significant differences in model outputs by subtly modifying the text, severely affecting the security and stability of the system ~\citep{wang2023punctuation, han2024bfs2adv}. These attacks not only reduce model accuracy, but can also lead to financial losses and legal risks ~\citep{fursov2021adversarial}.

Existing textual adversarial attacks can be categorized into white-box and black-box attacks ~\citep{baniecki2024adversarial}. White-box attackers have full access to all model information, including architecture and parameters~\citep{lin2021using}. Therefore, the attacker can obtain the gradient information to modify the input text to attack the model. 
% A more realistic scenario is a black-box attack, where the attacker does not have access to the model internals and can only execute the attack by accessing the training data or model outputs. \textcolor{red}{The former} is known as a transfer-based attack, an attack that relies on the availability of training data to train a suitable substitute model, attacking the victim model by exploiting the tranferability  of adversarial examples~\citep{kwon2022ensemble}. \textcolor{red}{The latter} is known as query-based attack, where the attacker relies on knowing the probability scores of the model outputs to optimize the adversarial text via a gradient free manner
A more practical scenario involves a black-box attack, where the attacker lacks access to the internal workings of the model and can instead perform the attack by either leveraging the training data or observing the model's outputs. The first approach, known as a transfer-based attack, involves using the available training data to train a substitute model and exploiting the transferability of adversarial examples to attack the victim model~\citep{kwon2022ensemble}. The second approach, referred to as a query-based attack, depends on obtaining the model's output probability scores to optimize the adversarial input in a gradient-free manner.~\citep{hu2024fasttextdodger,liu2024hqa,liu2023sspattack}.

Existing NLP models are usually deployed on Web pages through APIs~\citep{gonzalez2023improving}, and attackers cannot directly access the internal structure and parameter information of the models, making precise and efficient white-box attacks infeasible~\citep{inkawhich2020perturbing,wu2021improving,yuan2022adaptive,naseer2021generating,salman2020adversarially,deng2021adversarial}. In addition, for security reasons, such systems generally do not disclose detailed information about training data and outputs~\citep{li2020practical,sun2022towards,fang2022learning,jang2022strengthening,xie2019improving}, and probability scores~\citep{liu2024hqa}, to the user, and even prevent malicious cost by limiting the access frequency, thus further increasing the difficulty of black-box attacks~\citep{hu2024fasttextdodger}. To address this realistic challenge, we propose a novel attack hypothesis, \textit{i.e.}, can adversarial attacks still be effectively realized in the acknowledge of only the victim text?

We propose a real-world scenario-oriented attack method called the \textbf{Free Lunch Attack}  (FLA). The attack does not require knowledge of the structure of the victim model, training data, or even access to the victim model, and can be implemented relying only on the victim text. To achieve \textbf{zero access to the victim model}, we utilize publicly available pre-trained models to transform the victim text into vector representations and generate pseudo-labels through clustering to construct shadow datasets to train substitute models. However, due to the incomplete accuracy of the labeling of the shadow dataset, the substitute model obtained from the training is not sufficient to generate effective adversarial examples. To enhance the \textit{effectiveness of the attack}, we focus on balancing attack success rate (ASR) and operational efficiency. The Hierarchical Substitution Model Design incrementally aligns substitute models with the victim’s decision boundaries, enhancing ASR by refining the match over multiple iterations. Additionally, our Diverse Adversarial Example Generation strategy utilizes multiple attack methods to generate adversarial examples, minimizing the need for frequent retraining of models. This optimized process ensures a more efficient use of resources while maintaining high attack success.

In the text classification task, FLA is able to easily achieve an ASR of more than 40\%  at zero query cost, significantly undermining the predictive accuracy of the model. More importantly, FLA not only helps existing attack methods to improve the ASR by 34.99\% on average without additional queries, but also poses a far-reaching threat to mainstream Large Language Models (LLMs), such as  Qwen2, and the ChatGPT family, which can achieve up to 45.99\%  ASR. In addition, we deeply explore the attack efficacy of FLA with very few victimized samples or severe inconsistency with the training data distribution and show that even under these extreme conditions, FLA maintains an ASR more than 27.35\%. This demonstrates the highly destructive and indiscriminate nature of the attack against LLMs in real scenarios. \textbf{Meanwhile, FLA can achieve significant attack results even when only a small number of victim texts (\textit{e.g.}, $5$ texts) or merely the victim text attributes are available.}
Our main contributions can be summarized as follows:
% \begin{itemize}
%     \item We propose a novel attack scenario for text classification tasks, revealing the possibility that an attacker can exploit potential vulnerabilities to carry out an attack without accessing the model and without knowledge of its structure and training data. 
%     \item We design the Free Lunch Attack (FLA) framework, which successfully achieves an efficient attack on the model in a completely black-box environment by constructing a shadow training set and introducing gradient diversity. 
%     \item Experiments show that even the current state-of-the-art LLMs, such as  Qwen2, and the ChatGPT family, are not able to effectively defend against such attacks, highlighting the profound threat that FLA poses to model security. 
% \end{itemize}
\ding{182} We propose a novel attack scenario for text classification tasks, revealing the possibility that an attacker can exploit potential vulnerabilities to carry out an attack without accessing the model and without knowledge of its structure and training data. 
\ding{183} We design the Free Lunch Attack (FLA) framework, which successfully achieves an efficient attack on the model in a completely black-box environment by constructing a shadow training set and introducing gradient diversity. 
\ding{184} Experiments show that even the current state-of-the-art LLMs, such as  Qwen2, and the ChatGPT family, are not able to effectively defend against such attacks, highlighting the profound threat that FLA poses to model security. 


%-------------------------------------------------------------------------
\section{Related Work}\label{related-work}

\textbf{Text White-Box Attack:}
In a text white-box attack, attackers leverage complete knowledge of the victim model’s structure and parameters to generate adversarial examples. For instance, FD~\citep{papernot2016crafting} perturbs influential words based on the model’s gradient, while Hotflip~\citep{ebrahimi2018Hotflip} replaces words iteratively according to their importance score. TextBugger~\citep{ren2019generating} perturbs both characters and words using a greedy algorithm to maximize gradient disruption. \textit{However, the requirement for full model access limits the practicality of white-box attacks in real-world scenarios, where such information is generally unavailable.}

\textbf{Text Black-Box Attack:} In a text black-box attack, attackers generate adversarial examples without access to the model's internal structure, relying solely on input-output observations. Existing methods can be categorized into query-based and transfer-based attacks~\citep{waghela2024modified,han2024bfs2adv,zhu2024limeattack,kang2024hybrid}.
In query-based attacks, the attacker identifies important words based on the model’s output probabilities and targets them sequentially to alter the label. Examples include SememePSO~\citep{zang2020word}, which optimizes the search space using metaheuristics, and BAE~\citep{garg2020Bae}, which replaces words using BERT and prompt learning. Leap~\citep{xiao2023leap} speeds up convergence with adaptive particle swarm optimization, while HQA~\citep{liu2024hqa} minimizes perturbations by selecting optimal synonyms.
In transfer-based attacks, adversarial examples are generated on a substitute model and used to attack the victim model by exploiting model similarities. For instance, CT-GAT~\citep{lv2023ct} uses a sequence-to-sequence generative model to create adversarial examples across tasks. \textit{However, real-world systems often limit access to model details and frequencies, presenting new challenges for black-box attacks.}


In summary, the need for internal model information makes text white-box attacks challenging to implement in real-world scenarios, while restrictions on probability scores, substitute models, and query limits may hinder the effectiveness of black-box attacks. \textbf{In contrast, FLA is well-suited for more practical attack environments, as it can generate adversarial examples with high success rates even when only the victim texts or victim texts' topic is available.}
.


% (b)\textbf{No Interactive Access in Image Adversarial Attack} In the original 
% ``No Interactive Access''  scenario, attackers possess ample high-quality auxiliary data to train the substitute model and execute the transfer attack.~\citep{salman2020adversarially,deng2021adversarial,naseer2021generating,wu2021improving,yuan2022adaptive,inkawhich2020perturbing}. Then, some studies indicate that insufficient auxiliary data can also lead to successful attacks based on the training shallow substitute model\citep{li2020practical,sun2022towards}, input augmentation\citep{fang2022learning,jang2022strengthening,xie2019improving}, gradient stabilization\citep{wang2022enhancing,he2022boosting},
% better loss to train substitute model\citep{wang2021feature,li2020towards}, and 
% refine the substitute model\citep{xiaosen2023rethinking,yuan2021meta}. Recently, some work\citep{richards2021adversarial,inkawhich2021can} has shown that even with insufficient low-quality auxiliary data, attackers can perform adversarial attacks in``No Interactive Access''  scenario based on the better loss for the substitute model\citep{naseer2019cross,richards2021adversarial,huan2020data}.




% Within the context of the ``no-box'' approach in the CV domain, even if the attacker is denied access to the victim model, they can still obtain a small dataset from the same domain as the training set. This dataset comes with the soft label output of the victim model, thus allowing the attacker to acquire ground-truth information, even in a ``no-box'' scenario. In other scenarios related to ``no-box'' and ``No Interactive Access'', obtaining ground-truth information is also feasible. To the best of our knowledge, there has been no exploration of the impact of ground-truth information on text adversarial attacks.



\begin{figure*}
  \centering
  
  \includegraphics[width=0.78\textwidth]{figures/fla-flowchart-rev12-new.pdf} 
    % \vspace{-0.1in}
  \caption{\textbf{The Overview of FLA}. FLA utilizes a cluster-guided shadow dataset synthesis to create text-cluster label pairs for substitute model training. It then applies various attack methods to generate adversarial examples. If all adversarial examples fail to attack the substitute model, a new substitute model is trained to produce new adversarial examples. For successful attacks, if the maximum attack score \(S_{ig}\) exceeds the threshold \(\theta\), the highest-scoring example is chosen as the final adversarial example; otherwise, a new substitute model is required to generate new adversarial examples.
 }
 \label{overview}
  \vspace{-0.15in}
\end{figure*}





\section{Preliminary}
\ding{182}
\textbf{Victim Model}: The \textbf{victim model} refers to the target model that the attacker intends to attack, denoted as $f_v$. 
\ding{183}
 \textbf{Victim Text (Test Set)}: The \text{victim text (test set)} refers to the text that the attacker intends to modify. This is the text that the attacker is inevitably able to access. 
 \ding{184}
 \textbf{Substitute Model}: The substitute model approximates the decision boundary of the victim model and is used to generate adversarial samples, denoted as $f_{s}$ and $f_s(x) \approx f_v(x)$.
 \ding{185}
 \textbf{Shadow Dataset}: The shadow dataset refers to data that are accessible to the attacker. In victim text-only scenarios, the shadow dataset typically consists of unlabeled victim texts, such as those found in the test set. However, the shadow dataset does not necessarily need to be the test set; it only needs to share similar attributes. For example, in the 5-class sentiment analysis dataset SST5, the shadow dataset could be the unlabeled SST5 test set or an online sentiment dataset, like the binary Tomatoes dataset. As a result, the labels and data distribution in the shadow dataset may differ from those in the training dataset.
 \ding{186}
\textbf{Adversary’s Goals：}
Consider a text classification model $f_v$ that predicts labels $\hat{y} = \left[ C_1, C_2, \dots, C_m \right]$, where $m$ represents the total number of labels. At the same time, attackers only have access to victim texts, denoted $\{ x_1, x_2, \dots, x_n \}$, where $n$ corresponds to the number of victim texts.
Our goal is to generate adversarial examples $\{\tilde{x}_1^*,\tilde{x}_2^*, \dots ,\tilde{x}_n^*\}$ just based on victim texts $\{x_1, x_2, \dots, x_n\}$ and to successfully fool the victim model $f_v$, which aims at $f_v(x_i) \neq f_v(\tilde{x}_i^*)$.
% Let $D_s = \{(x_1, y_1), (x_2, y_2), \ldots, (x_m, y_m)\}$, where $x_i \in T_v$ and $y_i$ is the label generated by the victim model $f_v$ for the victim text $x_i$, \textit{i.e.}, $y_i = f_v(x_i)$. The shadow dataset is used to mimic the behavior of the victim model.
% \begin{equation}
% D_s = \{(x_i, f_v(x_i)) \mid x_i \in T_v\}
% \end{equation}

\section{Free Lunch Adversarial Attack}
To carry out the NLP model attack without access and understanding, we propose the Free Lunch Attack  (FLA), which creates a shadow dataset by generating cluster labels using K-means~\citep{lloyd1982least} clustering to achieve zero-access to the victim model. Next, we use the text-cluster label pairs to train the substitute model. Various attack methods are applied to generate adversarial examples. If all adversarial examples fail against the substitute model, a new substitute model is trained using the hierarchical substitution model design process. For the successful adversarial examples, we compute their attack scores. If the maximum attack score \(S_{ig}\) exceeds the threshold \(\theta\), the highest-scoring example is selected as the final adversarial example. Otherwise, a new substitute model, trained using the hierarchical substitution model design, is required to generate additional adversarial examples.



\subsection{Cluster-Guided Shadow Dataset Synthesis}\label{cluster-number}
% 步骤1：模拟影子数据。
% 问题：在没有训练数据的情况下，如何训练替代模型。
% 假设：受害者数据和训练数据分布相同(或者分布相似),给受害者文本打上伪标签，可以模仿训练数据，进而训练替代模型。
% 引用或证明：去找训练集和测试集同分布的假设论文来做引用。

Training a substitute model without access to the original training data poses a significant challenge in adversarial settings. This section proposes a method to synthesize a shadow training dataset by assigning pseudo-labels to victim texts.

We find that the victim data and training data exhibit similar distribution characteristics, a common supposition in machine learning suggesting that training and test sets follow the same distribution~\cite{zhu2019freelb}. Building on this, we hypothesize that texts eliciting strong responses from the model are likely akin to the training data, offering a viable proxy for estimating the training dataset.


To utilize victim texts effectively, we apply a clustering method to assign pseudo-labels to these unlabeled texts, thus creating a shadow dataset. As the Figure \ref{overview} shows,
 each victim text \(x_i\) is embedded using a pre-trained model \(f_{\text{pre}}\), denoted as \(\bm{E}(x_i) = f_{\text{pre}}(x_i)\). All victim text embeddings \(\bm{E} = [\bm{E}(x_1), \bm{E}(x_2), \dots, \bm{E}(x_n)]\) are then clustered into distinct groups, and cluster labels \(y_i^{\text{clu}}\) are assigned as pseudo-labels for each text. The resulting shadow dataset \(\bm{D}\) is defined as:

\begin{equation}
\bm{D}=\{(x_1, y_1^{\text{clu}}), (x_2, y_2^{\text{clu}}), \dots, (x_n, y_n^{\text{clu}})\}
\end{equation}
This dataset effectively approximates the distribution of the original training data, facilitating the training of the substitute model. Despite the discrepancies between victim data-pseudo label pairs and the original data-label pairs, which can hinder perfect alignment of the substitute model with the victim model's decision boundary, our aim is not to mirror the victim model but to develop a substitute model that can distinguish between classes clearly. The substitute model, trained on the shadow dataset \(\bm{D}\), while not an exact replica of the victim model, is adequate for conducting effective adversarial attacks. 





\begin{figure*}
  \centering
  \includegraphics[width=0.85\textwidth]{figures/fla-fig2-rev3-edition3.pdf} 
     \vspace{-0.15in}
  \caption{\textbf{The Overview of Hierarchical Substitution Model Design.} For the first iteration of FLA, all victim texts are employed to 
 train the substitute model $f_1^s$. For the second iteration, the victim texts with the positive cluster label $C_{\text{pos}}$ are employed to 
 train the substitute model $f_2^s$, the victim texts with the negtive cluster label $C_{\text{neg}}$ are employed to 
 train the substitute model $f_3^s$. Following this process, we can train the hierarchical substitution models.}
  \label{Overview-of-Hierarchical}
  \vspace{-0.15in}
\end{figure*}

\subsection{Hierarchical Substitution Model Design}
The substitute model trained in Section \ref{cluster-number} can clearly distinguish between classes, but it is not similar to the victim model, which compromises the effectiveness of the transfer attack. To address this, we propose a hierarchical training approach that aims to align substitute models more closely with the victim model's adversarial decision boundary.

Multiple substitute models are used to incrementally generate adversarial decision boundaries that progressively converge towards the victim model's boundary, enhancing the likelihood of a successful attack~\citep{papernot2016transferability}. This progressive alignment enhances the probability of a successful attack. Theorem \ref{max_prob1} formalizes this intuition.
\begin{theorem}\label{max_prob1}
As the number of substitute models $m$ increases, the probability of successfully attacking the victim model, denoted by $p_m^{\text{suc}}$, also increases, meaning:
\begin{equation}
\text{for } m > n, \quad p_m^{\text{suc}} > p_n^{\text{suc}}.
\end{equation}
\end{theorem}
\textit{Proof.} Please see Appendix \ref{number-of-substitute-models} for the proof. 

The process starts by training a substitute model, \(f_1^s\), using a shadow dataset \(\bm{D}\). Then, the shadow dataset is updated to train a new substitute model. As the Figure \ref{Overview-of-Hierarchical} shows, 
the whole process is as follows: \ding{182} For each victim text \(x_i\), we check its cluster label \(y_i^{\text{clu}}\). If this label corresponds to the positive cluster \(C_{\text{pos}}\), we include \(x_i\) in a new set of victim texts. \ding{183} After this, we obtain a new set of victim texts \(\{x_1^{\text{new}}, x_2^{\text{new}}, \dots, x_{n_1}^{\text{new}}\}\), where \(n_1 < n\), and each text has the positive cluster label \(C_{\text{pos}}\). \ding{184} Next, we perform a cluster-guided shadow dataset synthesis on this new set, assigning new cluster labels \(y_i^{\text{clu,new}}\) to each victim text \(x_i^{\text{new}}\). \ding{185} We update the shadow dataset \(\bm{D}_{\text{new}}\), which contains these newly labeled texts, and then use \(\bm{D}_{\text{new}}\) to train a new substitute model, \(f_1^s\). Similarly, for texts with negative cluster labels, we repeat this process to train another substitute model, \(f_2^s\).

By repeating this process \(u\) times, we generate \(U\) substitute models, where the total number of models is as follows:
\begin{equation}
    U = 2^0 + 2^1 + 2^2 + \dots + 2^u .
\end{equation}
Now, for each victim text \(x_i\), we apply the diverse adversarial example generation (Section \ref{Diverse}) to create an adversarial example \(\tilde{x}_i^{1}\). If this example fails to fool the current substitute model \(f_1^s\) (\textit{i.e.}, \(f_1^s(x_i) = f_1^s(\tilde{x}_i^{1})\)), we move on to the next substitute model, \(f_2^s\), and attempt to create a new adversarial example. This process continues until the adversarial example successfully attacks a substitute model, meaning \(f_j^s(x_i) \neq f_j^s(\tilde{x}_i^{1})\). The goal is to keep trying different substitute models until the attack is successful.

% We denote a text attack method by $M_1$.
% Specifically, we first employ the shadow dataset \(\bm{D}\) to 
% train the substitute model $f_1^s$.
% Next, we update the shadow dataset for training the new substitute model.   
% As illustrated in Figure \ref{Overview-of-Hierarchical}, for each victim text $x_i$, if its corresponding cluster label $y_i^{\text{clu}}$ is the positive cluster label $C_{\text{pos}}$, we include $x_i$ in the new set of victim texts. 
% After this process, we obtain a new set of victim texts denoted as
%  $\{{ x_1^{\text{new}}, x_2^{\text{new}}, \dots, x_{n_1}^{\text{new}} }\}$, where $n_1 < n$ and the cluster label of each $x_i^{\text{new}}$ is $C_{\text{pos}}$. Then, we employ the cluster-guided shadow dataset synthesis on this new set. In the cluster process of cluster-guided shadow dataset synthesis, we can obtain the new the cluster label  of $x_i^{\text{new}}$, denoted  as $y_{i}^{\text{clu,new}}$. Finally, we update the shadow dataset $\bm{D}_{\text{new}}$, defined as
% \begin{equation} \bm{D}_{\text{new}} = \{{(x_1^{\text{new}}, y_1^{\text{clu,new}}), (x_2^{\text{new}}, y_2^{\text{clu,new}}), \dots, (x_{n_1}^{\text{new}}, y_{n_1}^{\text{clu,new}})}\}. \end{equation}
% Then, we train the new substitute model $f_1^s$ based on $\bm{D}_{\text{new}}$. 
% Similarly, the victim texts with the negative cluster label are repeat the process of cluster-guided shadow dataset synthesis to train the new substitute model $f_2^s$.
% If we repeat this process 
% $u$ times, we can obtain $U$ substitute models, where 
% $U=2^0+2^1+2^2+\cdots+2^u.$
% For each victim text $x_i$, we employ $M_1$ to craft the corresponding adversarial example $\tilde{x}_i^{1}$, where $\tilde{x}_i^{1}=M_1(x_i, f_1^s)$. If $\tilde{x}_i^{1}$ cannot attack $f_1^s$, which means $f_1^s(x_i)=f_1^s(\tilde{x}_i^{1})$, the $x_i$ need to craft the adversarial example in new substitute model $f_2^s$. We repeat this process until the adversarial example of $x_i$ successfully attack the substitute model $f_j^s$, which means $\tilde{x}_i^{1}=M_1(x_i, f_j^s)$ and $f_j^s(x_i)\neq f_j^s(\tilde{x}_i^{1})$. 


\subsection{Diverse Adversarial Example Generation}\label{Diverse}
Training substitute models can be resource-intensive, especially when repeated iterations are required to generate effective adversarial examples. In each iteration, a new substitute model is trained on a subset of the shadow dataset, which is progressively reduced, limiting the available data for further training. Consequently, the continuous training of new substitute models becomes less feasible and increasingly costly. To address this, it is essential to evaluate the necessity of training additional substitute models and explore methods that minimize the associated training costs. 

This section proposes a strategy to reduce training expenses by utilizing diverse adversarial examples generated from multiple attack methods. Using multiple attack methods improves the chance of successfully attacking substitute models compared to relying on a single method. This reduces the costs of repeatedly training substitute models.

Consider \(w\) attack methods \(\{M_1, M_2, \dots, M_w\}\), each with success probabilities \(\{p_1, p_2, \dots, p_w\}\). The overall success probability is \(\max\{p_1, p_2, \dots, p_w\}\), which increases as more attack methods are employed. Theorem \ref{max_prob2} formalizes this intuition.

% Suppose $w$ attack methods, denoted as $\{M_1, M_2, \dots, M_w\}$, are used to target the substitute model, with the success probabilities for each method denoted as $\{p_1, p_2, \dots, p_w\}$. The success probability of a single method is $p_i$, while the success probability across all $w$ methods is $\max \{ p_1, p_2, \dots, p_w \}$. Thus, employing multiple attack methods to generate diverse adversarial examples increases the chances of success on the substitute model, which subsequently raises the probability of a successful attack on the victim model.

\begin{theorem}\label{max_prob2}
Suppose that $\{p_1, p_2, \dots, p_w\}$ be independent and identically distributed (\textit{i.i.d.})  success probabilities with cumulative distribution function (CDF) denoted by $F(p)$. Then as $w \to \infty$, the probability that $\max\{ p_1, p_2, \dots, p_w \} > p_i$ approaches $1$ for any $p_i < 1$. Formally,
\begin{small}
\begin{equation}
\begin{array}{c}
\lim\limits_{w \to \infty} \Pr\left( \max\{ p_1, p_2, \dots, p_w \} > p_i \right) = 1, \\
\lim\limits_{w \to \infty} \Pr\left( \max\{ p_1, p_2, \dots, p_w \} > \max\{ p_1, p_2, \dots, p_m \} \right) = 1, \\
 \text{for} \quad w > m. 
\end{array}
\end{equation}
\end{small}
\end{theorem}
\textit{Proof.} Please see Appendix \ref{Proof2} for the proof.

Theorem \ref{max_prob2} shows that as \(w \to \infty\), the probability of success approaches 1, indicating the benefit of using multiple attack methods to reduce training costs.
Take the substitute model \( f_1^s \) as an example, if an adversarial example \(\tilde{x}_i^{1} = M_1(x_i, f_j^s)\) fails to fool the model (i.e., \( f_1^s(x_i) = f_1^s(\tilde{x}_i^{1}) \)), this suggests a potential issue with either the one attack method \(M_1\) or the substitute model. Therefore, before deciding to train a new substitute model, we eliminate the influence of the failed attack method by employing multiple attack methods. Specifically, we use \( w \) attack methods \( \{ M_1, M_2, \dots, M_w \} \) to generate \( w \) adversarial examples:
\begin{equation}
\{\tilde{x}_i^{1}, \tilde{x}_i^{2}, \dots, \tilde{x}_i^{w}\}, \quad \text{where} \quad \tilde{x}_i^{j} = M_j(x_i, f_j^s).
\end{equation}
If none of these adversarial examples successfully fool \( f_1^s \), i.e., \( f_1^s(x_i) = f_1^s(\tilde{x}_i^{j}) \) for all \( j \), a new substitute model must be trained.


Among the successful adversarial examples, we select the one with the best attack performance, measured by the logit change of the substitute model currently in use and the similarity between \( x_i \) and the adversarial example \( \tilde{x}_i^j \). The attack performance score is:
\begin{equation}\label{adv}
s_{ij} = \alpha \left( o_{\hat{y}_i}(x_i) - o_{\hat{y}_i}(\tilde{x}_i^j) \right) + \beta \left( \frac{\bm{E}(x_i) \cdot \bm{E}(\tilde{x}_i^j)}{\|\bm{E}(x_i)\| \cdot \|\bm{E}(\tilde{x}_i^j)\|} \right),
\end{equation}
where $\left( o_{\hat{y}_i}(x_i) - o_{\hat{y}_i}(\tilde{x}_i^j) \right)$ is the logit change of the substitute model currently in use,
\( \alpha \) and \( \beta \) are scaling factors, and \( \bm{E}(x_i) \) and \( \bm{E}(\tilde{x}_i^j) \) are the embeddings.
The adversarial example with the highest score \( s_{ij} \) is selected as \( \tilde{x}_i^g \). If this score exceeds a threshold \( \theta \), \( \tilde{x}_i^g \) is accepted as the final adversarial example. Otherwise, a new substitute model is trained to generate a new adversarial example. 
}

\section{Experiment}
% \label{others}



\subsection{Experimental Setup}

\ding{182} \textbf{Datasets:} We perform primary experiments on the SST5 and Emotion datasets. The details of the datasets are presented in Appendix \ref{datasets}. 
\ding{183} \textbf{Metrics:}
Several metrics are used to evaluate the effectiveness of FLA, including Attack Success Rate (ASR), Cost, and Semantic Similarity (Sim) between the original texts and adversarial examples. 
% \textcolor{red}{The Cost metric measures the total number of queries, with one token required for each access.   ``need to explain more  why you use cost but not query?"}
We utilize the metric ``Cost" as it more accurately reflects real-world application scenarios. In this paper, \textbf{``Cost" is defined as the total number of queries made by the attack method to the model}, measured in units of ``tokens."
Detailed descriptions of these evaluation metrics are provided in Appendix \ref{em}.
\ding{184} \textbf{Substitute model:}
 The details of the substitute model are presented in Appendix \ref{surrogate-model}.
\ding{185}
\textbf{Baselines:}
\textbf{In the victim texts-only scenario, no prior work on attacks has been carried out. The stringent constraints of this scenario render all existing text attack methods ineffective. We have broadened the application conditions of other methods, enabling other text-attack algorithms to access any required information.} Several text attack methods are selected, including Bae~\citep{garg2020Bae},  FD~\citep{papernot2016crafting}, Hotflip~\citep{ebrahimi2018Hotflip}, PSO~\citep{zang2020word}, TextBug~\citep{ren2019generating}, Leap~\citep{xiao2023leap}, CT-GAT~\citep{lv2023ct}, and HQA~\citep{liu2024hqa}. The details of these methods are presented in Appendix \ref{baseline}. \textbf{ \uline{To ensure a fairer comparison, we restrict other attack methods to a maximum of $35$ accesses per victim text, as FLA does not access the victim model at all.}}
% For query-based methods, they obtain information through Cost on the victim model and determine the attack strategy. In the transfer attack, we access the victim text to the victim model to obtain the corresponding prediction label and train the substitute model. The details of training the substitute model are the same as FLA. We also employ the methods Bae~\citep{garg2020Bae}, FD~\citep{papernot2016crafting}, Hotflip~\citep{ebrahimi2018Hotflip}, and TextBug~\citep{ren2019generating} in the substitute model to generate adversarial examples. These samples are designed to deceive the victim models by leveraging their transferability.
\ding{186}
\textbf{Other Setup:}
The pre-trained embedding model ``T5"~\citep{raffel2020exploring} is effectively used to embed the victim texts and calculate their similarity. Furthermore, we apply the K--means clustering method to categorize the embedded texts.
The scaling factors $\alpha$ and $\beta$ in \eqref{adv} are set to $9$ and $1$, respectively. And 
the threshold \( \theta \)  is set to $4$.
FLA selects the Bae, FD, Hotflip, PSO, and TextBug as the attack methods. FLA conducts three rounds of iteration and trains eight substitute models.

% Our experiments were conducted on an A100 machine equipped with 80GB of memory.

% These methodologies utilize iterative techniques to generate candidate adversarial examples through repeated attacks on the victim model. However, our approach, which involves a limited number of Cost, restricts access to the victim model. To maintain a fair comparison, we have set a limit for the baseline attack algorithms to generate a maximum of 10
%  candidate adversarial examples for attacking the victim model.
% The documentation for \verb+natbib+ may be found at



\subsection{Comparison with Other Adversarial Attacks}\label{com_querry}


\begin{table*}[t]

\centering
\caption{The attack performance of FLA and adversarial attacks on Emotion and SST5 datasets.  For each metric, the best method is highlighted in \textbf{bold} and the runner-up is \underline{underlined}. }
\label{main-tab}
\resizebox{1\textwidth}{!}{

\begin{tabular}{@{}ccccccc|cccccc@{}}
\toprule
\multirow{3}{*}{Method} & \multicolumn{6}{c|}{SST5}                                        & \multicolumn{6}{c}{Emotion}                                     \\ \cmidrule(l){2-13} 
                        & \multicolumn{3}{c}{DistilBERT}    & \multicolumn{3}{c|}{RoBERTa} & \multicolumn{3}{c}{DistilBERT}    & \multicolumn{3}{c}{RoBERTa} \\ \cmidrule(l){2-13} 
                        & ASR(\%) \uparrow & Sim \uparrow & Cost \downarrow               & ASR(\%) \uparrow & Sim \uparrow & Cost \downarrow               & ASR(\%) \uparrow & Sim \uparrow & Cost \downarrow               & ASR(\%) \uparrow & Sim \uparrow & Cost \downarrow               \\ \midrule \midrule
 Bae& 42.71&     0.888 
& \multicolumn{1}{c|}{47360
} &        39.14   
&        0.887   
&            47466  
& 32.25 
&     0.926 
& \multicolumn{1}{c|}{43682
} &        32.95   
&        0.923  
&           43656  
\\
FD                      & 25.20 
&     0.939 
& \multicolumn{1}{c|}{27760
} &        22.30   
&        \textbf{0.982}&            21452  & 



22.30 
&     0.932 
& \multicolumn{1}{c|}{25612
} &        27.50    
&        \textbf{0.982}&           22850  
\\
 Hotflip& 41.50&     0.951 
& \multicolumn{1}{c|}{25455
} &        29.00   
&        0.951   
&            25956  
& 29.00 
&     0.949 
& \multicolumn{1}{c|}{28566
} &        28.05   
&        0.949  
&           28800  
\\
PSO                     & 45.14 
&     0.954 
& \multicolumn{1}{c|}{24398
} &        \underline{41.50}&        0.954   
&            27360  & 



39.50 
&     \underline{0.952}& \multicolumn{1}{c|}{23660
} &        \underline{37.65}&        0.951  
&           24190  
\\
 TextBug                 & 30.36&     \textbf{0.978}& \multicolumn{1}{c|}{69520
} &        20.85   
&        \underline{0.978}&            67009  
& 20.85 
&     \textbf{0.978}& \multicolumn{1}{c|}{60642
} &        21.45   
&        \underline{0.978}&           60662  \\
Leap                    & 32.55      
&     \underline{0.953}& \multicolumn{1}{c|}{\underline{21548}} &        30.07      
&        0.944               
&            \underline{21083}& 



40.58      
&     0.926               
& \multicolumn{1}{c|}{\underline{19460}} &        37.63      
&        0.911               
&           \underline{}19560\\
 CT-GAT                    & 
29.37&     0.939               
& \multicolumn{1}{c|}{46238            
} &        24.80      
&        0.926               
&            82957            
& 28.10      
&     0.904               
& \multicolumn{1}{c|}{52114            
} &        30.85      
&        0.906               
&           50686            
\\
 HQA                     & \underline{46.11}&     0.936               
& \multicolumn{1}{c|}{64855            
} &        39.64      
&        0.929               
&            64256            
& 



\underline{37.40}&     0.912               
& \multicolumn{1}{c|}{44876            
} &        
36.40      
&        0.911               
&           46326            
\\
\midrule \rowcolor{orange!50}  \textbf{FLA}                     & 
\textbf{52.08}&   0.950& \multicolumn{1}{c|}{\textbf{0}} &        \textbf{45.03}&       0.950&            \textbf{0}& \textbf{43.15}&     0.949& \multicolumn{1}{c|}{\textbf{0}} &       \textbf{42.05}&        0.949&          \textbf{0}\\ \bottomrule
\end{tabular}
}
\end{table*}
Table \ref{main-tab} presents the experimental results for both the SST5 and Emotion datasets. Our FLA method achieves state-of-the-art (SOTA) performance in both ASR and Cost metrics, demonstrating superior attack success rates with fewer queries. Notably, FLA delivers these results without querying the victim model or relying on any information regarding the model, ground truth, or training data. Regarding the similarity metric, while semantic similarity may be somewhat compromised during the hierarchical substitution model process, our diverse adversarial example generation method allows us to maintain a relatively high level of semantic similarity. 
\textbf{Additionally, other attack algorithms can improve the ASR by increasing query costs, but this improvement comes at the expense of a large number of queries, making them impractical for real-world applications. Meanwhile, we present the results without query limitations in the Appendix.}




% \begin{table*}[t!]
% \centering

% \caption{The ASR(\%) ↑ of hierarchical substitution model under different epochs setting  design. \textcolor{blue}{``Second Epoch'' and  ``Multiple Epoch'' indicate the attack under multiple iterative attacks, ``Query-based'' indicates the attack methods are normal attacks,} \textcolor{red}{maybe need more explain, what's difference betweeen "multiple iterative attacks" and "normal attack?" where's the point you want to show in this table?} ``Bae-FLA'', ``FD-FLA'', ``Hotflip-FLA'', ``PSO-FLA'', and ``TextBug-FLA'' indicate that transfer attack based on the substitute model generated by FLA method. For each metric, the best method is highlighted in \textbf{bold} and the runner-up is \underline{underlined}.    \textcolor{red}{ ``Query-based'' have been replace, need to update}}\label{Epoch-number}

% \resizebox{0.9\textwidth}{!}{ % 高度自动调
% \begin{tabular}{@{}cccccccccc@{}}
% \toprule
% Dataset                     & FLA's Variants & \begin{tabular}[c]{@{}c@{}}1st \\ itr \end{tabular} & \begin{tabular}[c]{@{}c@{}}2nd \\ itr\end{tabular} & \begin{tabular}[c]{@{}c@{}}Multiple \\ Epoch\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distil-\\ BERT\end{tabular} & \begin{tabular}[c]{@{}c@{}}1st \\ Epoch\end{tabular} & \begin{tabular}[c]{@{}c@{}}2nd \\ Epoch\end{tabular} & \begin{tabular}[c]{@{}c@{}}Multiple \\ Epoch\end{tabular} & RoBERTa \\ \midrule \midrule 
% \multirow{6}{*}{SST5}    & Bae-FLA&                                                        \textbf{35.20}&                                                       \textbf{40.72}&                                                          \textbf{46.38}&                                                       \underline{42.71}&                                                        \textbf{36.97}&                                                        \textbf{41.76}&                                                          \textbf{49.41}&                                                        \underline{39.14}\\
%                          & FD-FLA&                                                        20.54&                                                         29.91&                                                           22.62&                                                        25.20&                                                        20.50&                                                         24.21&                                                           23.71&                                                        22.30\\
%                          &Hotflip-FLA&                                                        24.71&                                                       25.88&                                                      33.89&                                                        41.50&                                                       23.53&                                                       24.66&                                                           32.99&                                                    29.00\\
%                          & PSO-FLA                 &                                                        \underline{26.06}&                                                         \underline{34.30}&                                                           34.12&                                                        \textbf{45.14}&                                                        24.16&                                                         28.28&                                                           29.23&                                                        \textbf{48.50}\\
%                          & TextBug-FLA&                                                        23.03&                                                         25.43&                                                           \underline{42.22}&                                                        30.36&                                                        19.41&                                                         21.09&                                                           33.54&                                                        20.85\\ \midrule
% \multirow{6}{*}{Emotion} & Bae-FLA
% &                                                        \textbf{25.55}&                                                         \textbf{30.80}&                                                           \textbf{42.50}&                                                        \underline{32.25}&                                                        \textbf{26.60}&                                                         \textbf{31.40}&                                                           \textbf{43.25}&                                                        \underline{32.95}\\
%                          & FD-FLA
% &                                                        20.05 &                                                         \underline{27.15}&                                                           31.65 &                                                        22.30 &                                                        20.90 &                                                         \underline{26.75}&                                                           32.30 &                                                        27.50  
% \\
%                          & Hotflip-FLA
% &                                                        19.40&                                                         19.95&                                                           28.05&                                                        29.00&                                                        17.85&                                                         18.60&                                                           26.85&                                                        28.05\\
%                          & PSO-FLA                 
% &                                                        \underline{20.85}&                                                         20.55 &                                                           29.00 &                                                        \textbf{48.50}&                                                        \underline{21.00}&                                                         20.15 &                                                           27.75 &                                                        \textbf{46.65}\\
%                          & TextBug-FLA
% &                                                        13.95&                                                         13.60&                                                           \underline{42.40}&                                                        20.85&                                                        14.05&                                                         13.50&                                                           39.25&                                                        21.45\\
%                          \bottomrule
% \end{tabular}

% }

% \end{table*}






\begin{figure}
  \centering
  \includegraphics[width=0.49\textwidth]{figures/hot4.pdf} 
    % \vspace{-0.1in}
  \caption{Experiment results under different clustering vectorization method. M1 and M2 represent DistilBERT and RoBERTa models for SST5, while M3 and M4 represent DistilBERT and RoBERTa models for Emotion. ``Avg'' denotes the mean score of ASR and similarity. \textbf{
The impact of clustering and vectorization methods on the attack effectiveness is random.}}\label{cluster-vector}
  \vspace{-10pt}
\end{figure}


% \begin{table}[t]
% \centering
% \caption{
% Experiment results of FLA under different few-shot data setting. ``ASR(\%) ↑'' indicates the attack success rate of victim models(Roberta and Distilbert).  \textcolor{blue}{``1'', ``2'', ``4'', ``8'' indicate the attack success rate of the few-shot data with 1,2,4,8 data in each label respectively, } \textcolor{red}{terrible expression problem, what does 1,2,4,8 mean? actual number? And ``1,2,4,8 indicates the success rate" experssion is wrong}  ``All'' indicates the victim texts are accessible. Even when the number of victim texts is limited, the FLA algorithm consistently achieves a notable ASR.}

% \label{few-shot}
% \resizebox{0.8\textwidth}{!}{%

% \begin{tabular}{@{}ccccccccccc@{}} 
% \toprule
%                                      & \multicolumn{5}{c}{Emotion}                                          & \multicolumn{5}{c}{SST5}                        \\ \midrule
% \multicolumn{1}{c|}{}                & 1       & 2       & 4       & 8       & \multicolumn{1}{c|}{All}     & 1       & 2       & 4       & 8       & All     \\ \midrule
% \multicolumn{1}{c|}{Roberta-ASR(\%) ↑}    & 27.55   & 29.75   & 30.15   & 33.25   & \multicolumn{1}{c|}{42.05}   & 39.28   & 41.27   & 37.51   & 38.51   & 45.03   \\ 
% \multicolumn{1}{c|}{Distilbert-ASR(\%) ↑} & 27.35   & 30.00   & 29.30   & 33.30   & \multicolumn{1}{c|}{43.15}   & 48.01   & 50.14   & 46.06   & 46.61   & 52.08   \\
% \multicolumn{1}{c|}{Sim↓}      & 0.929   & 0.923   & 0.923   & 0.916   & \multicolumn{1}{c|}{0.949}   & 0.901   & 0.897   & 0.902   & 0.905   & 0.950       \\ \bottomrule
% \end{tabular}

% }
% \end{table}


\begin{table}[t]
\centering
\caption{Few-shot attack performance of FLA on Emotion and SST5 datasets. \textbf{FLA can achieve significant ASR even in scenarios with very few victim texts. }}
\label{few-shot}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}c|ccc|ccc@{}}
\toprule
          & \multicolumn{3}{c|}{Emotion}                                                                                                        & \multicolumn{3}{c}{SST5}                                                                                                            \\ \midrule
Shot Size & \begin{tabular}[c]{@{}c@{}}Roberta\\ ASR(\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distilbert\\ ASR(\%) ↑\end{tabular} & Sim↓ & \begin{tabular}[c]{@{}c@{}}Roberta\\ ASR(\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distilbert\\ ASR(\%) ↑\end{tabular} & Sim↓ \\ \midrule  \midrule
1-shot    &                                                             27.55   &                                                                27.35   &      0.929   &                                                             39.28   &                                                                48.01   &      0.901   \\
2-shot    &                                                             29.75   &                                                                30.00   &      0.923   &                                                             41.27   &                                                                50.14   &      0.897   \\
4-shot    &                                                             30.15   &                                                                29.30   &      0.923   &                                                             37.51   &                                                                46.06   &      0.902   \\
8-shot    &                                                             33.25   &                                                                33.30   &      0.916   &                                                             38.51   &                                                                46.61   &      0.905   \\
Full-shot &                                                             42.05&                                                                43.15&      0.949&                                                             45.03   &                                                                52.08   &      0.950       \\ \bottomrule
\end{tabular}

\vspace{-10pt}

}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}



\subsection{Ablation Study }
% \subsubsection{The Impact of the Different clustering methods}
% \subsubsection{Different Clustering Method}
\ding{182} \textbf{Different Clustering Method:}
In this paper, the FLA method utilizes K-means as its clustering method. 
To mitigate the influence of different clustering methods, we introduce additional clustering methods, including Spectral clustering ~\citep{von2007tutorial}and BIRCH~\citep{zhang1996birch}.
The results are presented in Figure\ref{cluster-vector}. Subplots (a) and (b) of Figure\ref{cluster-vector} display the ASR and similarity metrics for various clustering methods. While the methods exhibit different levels of ASR and similarity between victim texts and models, the differences are not significant. \textbf{ \uline{Furthermore, no single method consistently achieves SOTA performance across all scenarios. These findings suggest that, although clustering methods can influence the effectiveness of the attack, the overall impact remains limited.}}
% \subsubsection{Different Vectorization Methods}
\ding{183} \textbf{Different Vectorization Methods}:
% \subsubsection{The Impact of the Different Vectorization Methods}
The ``T5'' pre-trained model is the vectorization method in FLA.
To mitigate the influence of different vectorization methods, we introduce additional vectorization methods, including CLIP~\citep{radford2021learning} and one-hot encoding~\citep{rodriguez2018beyond}. CLIP is a pre-trained model trained on an image-text pair dataset. In contrast, a one-hot encoding represents categorical data using a binary vector where an element is set to $1$ and all others are set to $0$. Unlike CLIP, one-hot encoding is not pre-trained and does not rely on any training data.
The results are presented in Figure\ref{cluster-vector}. The
subplots (c) and (d) of Figure\ref{cluster-vector} present the ASR and similarity of various vectorization methods. Although the methods show different levels of ASR and similarity between victim texts and models, the differences are not substantial. However, no single method consistently achieves SOTA performance in all scenarios. 
\begin{figure}
  \centering
  \includegraphics[width=0.33\textwidth]{figures/num4.pdf} % 替换为你的图片文件路径
  \caption{The ASR for different cluster numbers. \textbf{Fewer clusters imply better ASR.}}
  \label{cluster-number-fig}
  \vspace{-15pt}
\end{figure}
These results indicate that  
 \textbf{ \uline{while different vectorization methods influence the effectiveness of the attack, the overall impact is not substantial.}}
% \subsubsection{Different Cluster Number}
\ding{184} \textbf{Different Cluster Number}:
Based on the analysis in Section \ref{cluster-number}, using two clusters yields the optimal attack performance. Therefore, FLA implements two clusters in its approach. To evaluate the impact of different cluster numbers on attack 
performance, we conduct experiments with two, three, and four clusters. The primary evaluation metric is the Attack Success Rate (ASR). As shown in Figure \ref{cluster-number-fig}, the success rate decreases as the number of clusters increases. \textbf{ \uline{The highest success rate occurs with two clusters, validating our choice for FLA.}}






\subsection{Real-world Attack}
\subsubsection{Few-shot Victim Texts}
In few-shot victim texts scenario, 
 attackers only acquire a minimal portion of the victim texts. Specifically,  for each label in the SST5 and Emotion datasets, we select $1$, $2$, $4$, and $8$ victim texts respectively. 
 % During the cluster analysis phase, we select a clustering process in which both clusters are approximately 50\% to train the substitute model and implement transfer attacks. 
The ASR results for the few-shot data are presented in Table \ref{few-shot}. Even when each label is associated with only one text, the FLA algorithm still achieves ASR values of 27.55\%, 27.35\%, 39.28\%, and 48.01\%, respectively. Notably, in the SST5 dataset, a decrease in the number of victim texts does not significantly reduce the ASR. 
Notably, with very few samples, fewer samples can sometimes yield better attack results. This indicates that when the sample size is extremely small, the ASR fluctuates significantly. Meanwhile,
a decrease in the number of victim texts leads to a reduction in similarity; however, this decline progresses at a relatively slow rate.
\textbf{ \uline{Our results indicate that even with a very limited amount of victim texts, FLA can successfully attack the victim model.}}

\subsubsection{ Zero-shot Victim Texts }
In previous experiments, we assume that the attacker can access to the victim texts. However, we now investigate a scenario known as the \textbf{zero-shot data} scenario, in which the attacker does not have access to the victim texts. In this case, although the attacker lacks direct access to the victim texts, they are aware of key attributes. Specifically, the attacker knows that the victim texts are related to an emotion classification task. Leveraging this information, the attacker gathers similar sentiment analysis datasets from the Internet, such as Go-Emotions \citep{Goemotion} and Rotten Tomatoes \citep{Pang+Lee:05a}. We then apply FLA to these datasets to train the substitute model. The results, presented in Table \ref{Zero-shot-Data}, show that without access to the victim texts or model, FLA still achieves an ASR of over 30\%. For example, on the SST5 dataset, when DistilBERT is used as the victim model and Go-emotion data is applied, the ASR even reaches 50.36\%, almost identical to the 50.36\% achieved using SST5 victim texts directly. In the zero-shot data scenario, although the ASR decreases, it remains significantly high. However, compared to the ASR, the zero-shot data scenario exerts a more pronounced negative effect on similarity.
In summary, our findings suggest that \textbf{ \uline{an attack remains viable even without direct access to the victim texts, as long as the datasets used share similar attributes.}}

% Please add the following required packages to your document preamble:
% \usepackage{graphicx}







% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{graphicx}
% \begin{table}[t]
% \centering
% \caption{Experiment results of FLA under zero-shot data.``ASR(\%) ↑'' indicates the attack success rate of victim models(Roberta and Distilbert).  ``Go-emotion '', ``Tomatoes'', ``Emotion'', ``SST5'' indicate the datasets to train the substitute model respectively, 
% ``Roberta-ASR'' indicates the attack success rate of the Roberta model, ``Distilbert-ASR'' indicates the attack success rate of the Distilbert model. 
% % ``Cost'' indicates the total number of Cost, and ``Similarity'' indicates the average semantic similarity of original texts and adversarial texts.
% }
% \label{Zero-shot-Data}
% \resizebox{0.85\textwidth}{!}{%
% \begin{tabular}{@{}c|ccc|ccc@{}}
% \toprule
%            & \multicolumn{3}{c|}{Emotion}    & \multicolumn{3}{c}{SST5}        \\ \midrule
%            & Go-emotion & Tomatoes  & Emotion & Go-emotion & Tomatoes  & SST5    \\ \midrule \rowcolor{gray!20}
% Roberta-ASR(\%) ↑    & 30.15     & 31.05   & 42.05   & 39.46     & 40.00   & 45.03   \\
% Distilbert-ASR(\%) ↑ & 33.60     & 32.45   & 43.15   & 50.36     & 49.82   & 52.08   \\ \rowcolor{gray!20}
% Similarity     & 0.932     & 0.927   & 0.949   & 0.911     & 0.909   & 0.950   \\ 
% \bottomrule
% \end{tabular}
% }
% \end{table}


\begin{table}[t]
\centering
\caption{Zero-shot attack performance of FLA.
The attackers cannot access the victim texts, but only knows the sentiment-related text of the victim. Therefore, it collects sentiment-related texts, like the Go-emotion or Rotten Tomatoes datasets. \textbf{FLA can achieve significant ASR even without accessing the victim texts.}}

\label{Zero-shot-Data}
\resizebox{0.48\textwidth}{!}{%
\begin{tabular}{@{}ccccc@{}}
\toprule
Victim   Dataset    & Access Dataset & \begin{tabular}[c]{@{}c@{}}Roberta\\ ASR(\%) ↑\end{tabular} & \begin{tabular}[c]{@{}c@{}}Distilbert\\ ASR(\%) ↑\end{tabular} & Sim↓ \\ \midrule \midrule
\multirow{3}{*}{SST5}& Go-emotion & 39.46     & 50.36     & 0.911     \\
                   & Tomatoes  & 40.00   & 49.82   & 0.909   \\
                   & SST5& 45.03   & 52.08   & 0.950   \\ \midrule
\multirow{3}{*}{Emotion}& Go-emotion 
& 30.15     & 33.60     & 0.932     \\
                   & Tomatoes  
& 31.05   & 32.45   & 0.927   \\
                   & Emotion & 42.05   & 43.15   & 0.949   \\ \bottomrule
\end{tabular}
}
\vspace{-20pt}
\end{table}


% \setlength{\intextsep}{0pt}  % 减少图表与正文之间的上下间距
% \setlength{\columnsep}{10pt}  % 设置图表与文本之间的水平间距




\subsubsection{LLMs Attack}
We also discuss the effectiveness of FLA in LLMs, including Qwen2~\citep{yang2024qwen2}, ChatGPT4o and ChatGPT4omini~\citep{openai2023chatgpt4}, by
comparing the effectiveness of FLA and transfer attacks. We construct agents using LLMs through prompt learning. Below is our prompt template, using the Emotion dataset as an example: prompt ''The objective is to predict the label of the provided text. It is sufficient to supply the label alone. The labels encompass ‘Anger’, ‘Fear’, ‘Joy’, ‘Love’, ‘Sadness’, and ‘Surprise’, excluding any other classifications."
In closed-source LLMs and prompt-based learning scenarios, where gradients and label probabilities are unavailable, our baseline shows that CT-GAT is capable of launching an attack. Consequently, we compare the attack performance of CT-GAT with that of FLA.
Table \ref{llm} displays the experimental results for LLMs. 
Surprisingly, FLA achieves an attack success rate of over 27\% across all datasets and state-of-the-art LLMs, even with only limited access to the victim texts. \textbf{ \uline{These results indicate that an attacker can successfully target closed-source large language models with access to only the victim texts.}}



\subsection{Other experiments}
\ding{182} \textbf{The Impact of Substitute Model Quantity on Attack Effectiveness}:
\begin{table}[t]
\caption{The ASR of FLA's variants with  different substitute model quantity .  
``Bae-FLA'', ``FD-FLA'',
``Hotflip-FLA'', ``PSO-FLA'', and ``TextBugger-FLA'' indicate that transfer attack based on the substitute model generated by FLA method. These attacks are implemented by Bae, FD, Hotflip, PSO, and
TextBugger methods.}\label{Epoch-number}
\resizebox{0.49\textwidth}{!}{ % 高度自动调
\begin{tabular}{@{}cc|ccc|ccc@{}}
\toprule
\multirow{3}{*}{\rotatebox[origin=c]{90}{Dataset}} & \multirow{3}{*}{FLA's Variants}& \multicolumn{3}{c|}{DistilBERT}                                                                                                                                             & \multicolumn{3}{c}{RoBERTa}                                                                                                                                                 \\ \cmidrule(l){3-8} 
                         &                        & \begin{tabular}[c]{@{}c@{}}1 Model \\ Used\end{tabular} & \begin{tabular}[c]{@{}c@{}}3 Models\\ Used\end{tabular} & \begin{tabular}[c]{@{}c@{}}8 Models\\ Used\end{tabular} & \begin{tabular}[c]{@{}c@{}}1 Model \\ Used\end{tabular} & \begin{tabular}[c]{@{}c@{}}3 Models\\ Used\end{tabular} & \begin{tabular}[c]{@{}c@{}}8 Models\\ Used\end{tabular} \\ \midrule\midrule
\multirow{5}{*}{\rotatebox[origin=c]{90}{SST5}}    & Bae-FLA
& \textbf{35.20}& \textbf{40.72}& \textbf{46.38}
& \textbf{36.97}& \textbf{41.76}& \textbf{49.41}
\\
                         & FD-FLA
& 20.54& 29.91& 31.27
& 20.50& 24.21& 23.71
\\
                         & Hotflip-FLA
& 24.71& 25.88& 33.89
& 23.53& 24.66& 32.99
\\
                         & PSO-FLA                 
& \underline{26.06}& \underline{34.30}& 34.12
& \underline{24.16}& \underline{28.28}& 29.23
\\
                         & TextBug-FLA& 23.03& 25.43& \underline{42.22}
& 19.41& 21.09& \underline{33.54}\\ \midrule 
\multirow{5}{*}{\rotatebox[origin=c]{90}{Emotion}} & Bae-FLA
& \textbf{25.55}& \textbf{30.80}& \textbf{42.50}
& \textbf{26.60}& \textbf{31.40}& \textbf{43.25}
\\
                         & FD-FLA
& 20.05 & \underline{27.15}& 31.65 
& 20.90 & \underline{26.75}& 32.30 
\\
                         & Hotflip-FLA
& 19.40& 19.95& 28.05
& 17.85& 18.60& 26.85
\\
                         & PSO-FLA                 
& \underline{20.85}& 20.55 & 29.00 
& \underline{21.00}& 20.15 & 27.75 
\\
                         & TextBug-FLA& 13.95& 13.60& \underline{42.40}& 14.05& 13.50& \underline{39.25}\\ \bottomrule 
\end{tabular}

}

\end{table}
\begin{figure}
  \centering

  \includegraphics[width=0.47\textwidth]{figures/wo3.pdf} % 替换为你的图片文件路径
  \caption{The ASR of FLA with and without the defense method. ``W" indicates the FLA with the defense method. And ``W/O" indicates the FLA without the defense method.
  \vspace{-10pt}
}\label{defense-results}

   \vspace{-10pt}
\end{figure}
To examine the effect of the number of substitute models on attack performance, we created scenarios using  $1$, $3$, and $8$ substitute models. Furthermore, to eliminate the impact of varying attack algorithms, we applied only a single attack algorithm in each scenario. The results are presented in Table \ref{Epoch-number}, 
employing more substitute models leads to a gradual increase in ASR, at times even surpassing the performance of directly applying the attack method to the victim model. For example, when the victim texts are SST5 and the victim model is DistilBERT, the TextBug method achieves a 30.36\% ASR on the victim model while using TextBug with $7$ substitute models increases the ASR to 42.22\%.
\textbf{ \uline{The results suggest that increasing the number of substitute models can enhance attack performance.}}
\ding{183} \textbf{Attack Results under Defense Method}:
Adversarial training is a widely used  defense mechanism~\citep{qiu2019review}; however,    defense mechanism~\citep{qiu2019review};
however,  retraining models using this approach is resource-intensive. Therefore, training-free defense methods are more appropriate 
for FLA. In this work, we adopt the defense method proposed by \citep{wang2023punctuation} and apply prompt learning on large language models (LLMs) to mitigate adversarial text inputs. As shown in Figure \ref{defense-results}, \textbf{ \uline{the ASR decreases significantly after applying this defense, though the attack remains partially effective.}} Meanwhile, we present the results of adversarial training in the appendix.
\ding{184} \textbf{Further Experimental Results on Additional Datasets}:
To further explore the attack effectiveness of FLA, we conducted experiments on two additional datasets: Agnews~\citep{Zhang2015CharacterlevelCN} and TREC6~\citep{voorhees2000overview}. FLA demonstrated strong attack performance across both datasets.  Detailed results are presented in Table \ref{More-data-results} in appendix \ref{more-result},  FLA achieves zero queries, the best results among all approaches. In DistilBert victim model, FLA's ASR outperformed the second-best method by 4\% on Agnews, and 8.08\% on TREC6. 
When RoBERTa is used as the victim model, FLA also achieves SOTA attack results.
These results demonstrate that FLA effectively attacks a diverse range of datasets.



\begin{table}[t]

\centering
\caption{The ASR(\%)↑ of LLMs.
}
\label{llm}
\resizebox{0.49\textwidth}{!}{

\begin{tabular}{@{}c|ccc|ccc@{}}
\toprule
Dataset      & \multicolumn{3}{c|}{SST5} & \multicolumn{3}{c}{Emotion} \\ \midrule
Victim Model & GPT4o & GPT4omini & Qwen2 & GPT4o  & GPT4omini  & Qwen2 \\ \midrule \midrule
CT-GAT       & 20.23 & 19.85     & 27.36 & 16.15  & 17.85      & 24.20 \\
FLA          & 35.37 & 36.91     & 45.99 & 27.65  & 29.30       & 36.35 \\ \bottomrule

\end{tabular}

}
\vspace{-10pt}

\end{table}






















\section{Conclusion }
We present a novel scenario called the victim texts-only scenario and the corresponding approach, referred to as FLA. Our study is the first to demonstrate that text adversarial attacks do not require information about the victim model, labeling, or auxiliary data. Attackers can generate adversarial examples using only the victim texts.  \textbf{
Both few-shot and zero-shot scenarios demonstrate that adversarial examples can still be generated with limited victim texts and minimal attribute knowledge.}
To the best of our knowledge, the victim texts-only scenario represents the most stringent attack scenario for adversarial examples.
% Meanwhile, If an attack method succeeds in this scenario, it is likely to succeed in other attack scenarios as well. Because victim texts-only scenario requires the least amount of information, which makes it the most challenging. In contrast, other scenarios offer more information.
% Meanwhile,  we also look forward to the application of FLA in other modalities. FLA functions as a plug-and-play framework, requiring only a publicly available pre-trained model. 
If an attack method succeeds in this scenario, it is likely to succeed in others, as the victim-only text scenario requires the least information, making it the most challenging. Other scenarios, offering more data, may be easier to exploit.
We are excited about the potential applications of FLA in other modalities. FLA serves as a plug-and-play solution, \textit{requiring only a publicly available pre-trained model.} Pre-trained models such as CLIP for images, Wav2Vec for speech, and VideoBERT for video are readily available, making FLA suitable for tasks in these modalities. \textbf{Additional results, proofs, and details are provided in the appendix. Please refer to these for further insights.}


% \subsection{Dual submission}

% Please refer to the author guidelines on the \confName\ \confYear\ web page for a
% discussion of the policy on dual submissions.

% \subsection{Paper length}
% Papers, excluding the references section, must be no longer than eight pages in length.
% The references section will not be included in the page count, and there is no limit on the length of the references section.
% For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
% {\bf There will be no extra page charges for \confName\ \confYear.}

% Overlength papers will simply not be reviewed.
% This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
% Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
% The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
% The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

% %-------------------------------------------------------------------------
% \subsection{The ruler}
% The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
% The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
% If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
% The presence or absence of the ruler should not change the appearance of any other content on the page.
% The camera-ready copy should not contain a ruler.
% (\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

% Reviewers:
% note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
% Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


% \subsection{Paper ID}
% Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
% If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


% \subsection{Mathematics}

% Please number all of your sections and displayed equations as in these examples:
% \begin{equation}
%   E = m\cdot c^2
%   \label{eq:important}
% \end{equation}
% and
% \begin{equation}
%   v = a\cdot t.
%   \label{eq:also-important}
% \end{equation}
% It is important for readers to be able to refer to any particular equation.
% Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
% It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
% (Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
% All authors will benefit from reading Mermin's description of how to write mathematics:
% \url{http://www.pamitc.org/documents/mermin.pdf}.

% \subsection{Blind review}

% Many authors misunderstand the concept of anonymizing for blind review.
% Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

% Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
% That is all.
% (But see below for tech reports.)

% Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
% it says that you are building on her work.
% If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

% An example of a bad paper just asking to be rejected:
% \begin{quote}
% \begin{center}
%     An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Removed for blind review
% \end{quote}


% An example of an acceptable paper:
% \begin{quote}
% \begin{center}
%      An analysis of the frobnicatable foo filter.
% \end{center}

%    In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
%    Why the previous paper was accepted without this analysis is beyond me.

%    [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
% \end{quote}

% If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
% In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
% \begin{quote}
% [1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
% \end{quote}

% Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
% For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
% Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
% Then submit the tech report as supplemental material.
% Again, you may not assume the reviewers will read this material.

% Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
% For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
% solution.
% The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

% You can handle this paper like any other.
% Do not write ``We show how to improve our previous work [Anonymous, 1968].
% This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
% That would be silly, and would immediately identify the authors.
% Instead write the following:
% \begin{quotation}
% \noindent
%    We describe a system for zero-g frobnication.
%    This system is new because it handles the following cases:
%    A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
%    Ours handles it by including a foo term in the bar integral.

%    ...

%    The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
%    It displayed the following behaviours, which show how well we solved cases A and B: ...
% \end{quotation}
% As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
% A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
% He or she would have to be sure that no other authors could have been contracted to solve problem B.
% \medskip

% \noindent
% FAQ\medskip\\
% {\bf Q:} Are acknowledgements OK?\\
% {\bf A:} No.  Leave them for the final copy.\medskip\\
% {\bf Q:} How do I cite my results reported in open challenges?
% {\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
% For your results, however, you should not identify yourself and should not mention your participation in the challenge.
% Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

% \begin{figure}[t]
%   \centering
%   \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
%    %\includegraphics[width=0.8\linewidth]{egfigure.eps}

%    \caption{Example of caption.
%    It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
%    \label{fig:onecol}
% \end{figure}

% \subsection{Miscellaneous}

% \noindent
% Compare the following:\\
% \begin{tabular}{ll}
%  \verb'$conf_a$' &  $conf_a$ \\
%  \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
% \end{tabular}\\
% See The \TeX book, p165.

% The space after \eg, meaning ``for example'', should not be a sentence-ending space.
% So \eg is correct, {\em e.g.} is not.
% The provided \verb'\eg' macro takes care of this.

% When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
% If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
% However, use it only when there are three or more authors.
% Thus, the following is correct:
%    ``Frobnication has been trendy lately.
%    It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
%    Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

% This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

% \begin{figure*}
%   \centering
%   \begin{subfigure}{0.68\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{An example of a subfigure.}
%     \label{fig:short-a}
%   \end{subfigure}
%   \hfill
%   \begin{subfigure}{0.28\linewidth}
%     \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
%     \caption{Another example of a subfigure.}
%     \label{fig:short-b}
%   \end{subfigure}
%   \caption{Example of a short caption, which should be centered.}
%   \label{fig:short}
% \end{figure*}

